ViGoR: Improving Visual Grounding of Large Vision Language Models with Fine-Grained Reward Modeling

By combining natural language understanding, generation capabilities, and breadth of knowledge of large language models with image perception, recent large vision language models (LVLMs) have shown unprecedented visual reasoning capabilities. However, the generated text often suffers from inaccurate grounding in the visual input, resulting in errors such as hallucination of nonexistent scene elements, missing significant parts of the scene, and inferring incorrect attributes of and relationships between objects. To address these issues, we introduce a novel framework, ViGoR (Visual Grounding Through Fine-Grained Reward Modeling) that utilizes fine-grained reward modeling to significantly enhance the visual grounding of LVLMs over pre-trained baselines. This improvement is efficiently achieved using much cheaper human evaluations instead of full supervisions, as well as automated methods. We show the effectiveness of our approach through a variety of evaluation methods and benchmarks. Additionally, we released our human annotation (https://github.com/amazon-science/vigor) comprising 15,440 images and generated text pairs with fine-grained evaluations to contribute to related research in the community.

==> algorithms/auto_score.tex <==
\begin{algorithm}[t]
\caption{Automatic Method Reward Model Score}
\begin{algorithmic}[1]
\State \textbf{Input:} $Image$, \{\textit{Descriptions}\}, Perception Model $R_A$
    \For{each $S_i$ in \{\textit{Descriptions}\}}
        % \State Divide $S_i$ into a set of sentences $\{s_{i,1}, s_{i,2}, \ldots, s_{i,m}\}$
        \State $P^a_i \gets 0$
        \State $N^a_i \gets 0$
        \For{each noun phrase $n_{i,j}$ in $S_i$}
            \If{$n_{i,j}$ is detected by $R_A$}
                \State $P_i^a \gets P^a_i + 1$
            \Else
                \State $N_i^a \gets N^a_i + 1$
            \EndIf
        \EndFor
        \State The final scores for $S_i$ are $(N^a_i, P^a_i)$
    \EndFor
\end{algorithmic}
\label{alg:auto}
\end{algorithm}



% \State \textbf{Input:} $Image$, \{\textit{Descriptions}\}, Trained Reward Model $R_H$
%     \For{each $S_i$ in \{\textit{Descriptions}\}}
%         \State Divide $S_i$ into a set of sentences $\{s_{i,1}, s_{i,2}, \ldots, s_{i,m}\}$
%         \State $P^h_i \gets 0$
%         \State $N^h_i \gets 0$
%         \For{each sentence $s_{i,j}$ in $\{s_{i,1}, s_{i,2}, \ldots, s_{i,m}\}$}
%             \If{$R_H(s_{i,j}, \{s_{i,1}, s_{i,2}, \ldots, s_{i,j-1}\}, Image)$ = 0}
%                 \State $P^h_i \gets P^h_i + 1$
%             \Else
%                 \State $N^h_i \gets N^h_i + 1$
%             \EndIf
%         \EndFor
%         \State The final scores for $S_i$ are $(N^h_i, P^h_i)$
%     \EndFor

==> algorithms/human_score.tex <==
\begin{algorithm}
\caption{Human Feedback Reward Model Score}
\begin{algorithmic}[1]

\footnotesize

\State \textbf{Input:} $Image$, \{\textit{Descriptions}\}, Trained Reward Model $R_H$
    \For{each $S_i$ in \{\textit{Descriptions}\}}
        \State Divide $S_i$ into a set of sentences $\{s_{i,1}, s_{i,2}, \ldots, s_{i,m}\}$
        \State $P^h_i \gets 0$
        \State $N^h_i \gets 0$
        \For{each sentence $s_{i,j}$ in $\{s_{i,1}, s_{i,2}, \ldots, s_{i,m}\}$}
            \If{$R_H(s_{i,j}, \{s_{i,1}, s_{i,2}, \ldots, s_{i,j-1}\}, Image)$ = 0}
                \State $P^h_i \gets P^h_i + 1$
            \Else
                \State $N^h_i \gets N^h_i + 1$
            \EndIf
        \EndFor
        \State The final scores for $S_i$ are $(N^h_i, P^h_i)$
    \EndFor
\end{algorithmic}
\label{alg:human}
\end{algorithm}

==> figures/automatic_model.tex <==
\begin{figure}[t]
    \centering
    \includegraphics[width=0.8\linewidth]{images/automatic_model.pdf}
    \caption{\textbf{Illustration of reward modeling with automatic methods.}}
    \label{fig:automatic_model}
\end{figure}

==> figures/mmvig.tex <==
\begin{figure*}
    \centering
    \includegraphics[width=0.8\linewidth]{images/mmvig.pdf}
    \caption{\textbf{MMViG benchmark examples.}}
    \label{fig:mmvig}
\end{figure*}

==> figures/preliminary.tex <==
\begin{figure}
    \centering
    \includegraphics[width=\linewidth]{images/preliminary.pdf}
    \caption{A general framework of Large Vision Language Model.}
    \label{fig:framework}
\end{figure}

==> figures/rejection.tex <==
\begin{figure}
    \centering
    \includegraphics[width=0.8\linewidth]{images/rejection.png}
    \caption{\textbf{Illustration of the rejection sampling procedure.}}
    \label{fig:rejection}
\end{figure}



==> sections/1_intro_old.tex <==
\section{Introduction}
\label{sec:intro}

Large language models (LLMs) have garnered intense interest throughout the research and academic communities. These are usually pre-trained with tremendous amounts of automatically aggregated text data and further fine-tuned with specific user examples or evaluation feedback to enable the models to follow human-provided prompts and retrieve useful relevant information or solve logical problems. Recently, numerous techniques have augmented these breakthroughs with the capability of understanding image information by further injecting image features into the prompt encoding process. Unfortunately, large vision language models (LVLM) are often observed to generate dialogue that is more driven by the regularities learned by the text decoder rather than being solidly grounded in the factual content of the underlying image. 

While strong contextual grounding of language-only models can be learned from the enormous corpus of text data, training data for multimodal language / vision models is much more limited and flawed, while the complexity of the task is arguably higher. High-quality paired language / image datasets are typically relatively small and expensive to collect (such as VQA, OCR, TextCaps, etc.). Large, automatically compiled datasets, such as the LAOIN-5B dataset, tend to feature only simple images with very short text descriptions. To overcome these issues, there have been attempts (such as LLaVA) to semiautomatically generate reference dialogues, which nonetheless can create nonfactual statements such as hallucinations and omissions. 

\input{figures/teaser}

To address these issues in both LLMs and LVLMs, numerous recently proposed techniques train reward models to evaluate sampled output text and provide a score with which the base model can be fine-tuned by learning from human preference feedback. This is typically done by asking humans to compare two generated results holistically~\cite{llama2}. However, in \cite{uesato2022process}, the authors show that by training with dense supervision for each subcomponent of the generated text of an LLM, the reward model learns to more effectively guide the base model toward generating results that are correct at every step, rather than simply being correct as the final result. Inspired by this, we derive fine-grained information from both human annotators and automated methods to create supervision signals for the cross-modality use case. We show that this strategy can leverage the latest advances in perception models, as well as efficiently use human annotator effort to robustly improve visual grounding of LVLMs. 

In summary, our contributions are threefold. 

\begin{itemize}
    \item We show a framework for using a small quantity of human evaluation data to train a reward model to evaluate the generated results of LVLMs and efficiently incorporate human feedback into LVLM fine-tuning through rejection sampling.
    \item We further show that existing large open-set perception models can be leveraged to increase the factual grounding of LVLMs without additional human effort. 
    \item We create and plan to release the human evaluation dataset comprising 16k pairs of image and generated results, along with per-sentence evaluation annotation providing detailed quality assessments. 
\end{itemize}

==> tables/ablation.tex <==
\begin{table}[t]
\hspace*{0.05\textwidth}
\begin{minipage}[t]{.27\linewidth}
    \centering
    \begin{tabular}{cccc}
         \textbf{AT} & \textbf{HF} & \textbf{RF} & MMViG\\
        \midrule
        \cmark & - & - & \\
        \cmark & \cmark & - & - \\
        \cmark & \cmark & \cmark & 575.31 \\
    \end{tabular}
    \caption*{(a)}
    \label{tab:ab_aug}
\end{minipage}
\hspace*{0.05\textwidth}
\begin{minipage}[t]{.27\linewidth}
    \centering
    \begin{tabular}{lc}
         \textbf{reward model design} & MMViG\\
        \midrule
        none & -\\
        outcome-based & - \\
        fine-grained-based & - \\
    \end{tabular}
    \caption*{(b) }
    \label{tab:ab_aug}
\end{minipage}

\caption{\textbf{Ablation studies of our design choices}. We report the overall performance on MMViG benchmark. Please refer to Sec~\ref{sec:ablation} for a detailed analysis.}
\label{tab:ablation}
\end{table}

==> tables/ablation_backup.tex <==
\begin{table*}[t]
\hspace*{0.05\textwidth}
\begin{minipage}[t]{.27\linewidth}
    \centering
    \begin{tabular}{lc}
         \textbf{reward signal} & MMViG\\
        \midrule
        none & -\\
        fake object & -\\
        inaccurate attribute & -\\
        inaccurate relation & -\\
        inaccurate reasoning & -\\
        missing objects & -\\
        all & \\
    \end{tabular}
    \caption*{(a)}
    \label{tab:ab_depth}
\end{minipage}
\hspace*{0.05\textwidth}
\begin{minipage}[t]{.27\linewidth}
    \centering
    \begin{tabular}{lc}
         \textbf{reward model design} & MMViG\\
        \midrule
        none & -\\
        outcome-based & -\\
        fine-grained-based & -\\
    \end{tabular}
    \caption*{(b) }
    \label{tab:ab_aug}
\end{minipage}
\hspace*{0.05\textwidth}
\begin{minipage}[t]{.27\linewidth}
    \centering
    \begin{tabular}{lc}
     Module & MMViG \\
        \midrule
        none & -\\
        hallucination & -\\
        counting & -\\
        attribute & -\\
        all & -\\
    \end{tabular}
    \caption*{(c)}
    \label{tab:ab_ratio}
\end{minipage}

\caption{\textbf{Ablation studies of our design choices}. We report the overall performance on MMViG benchmark. Please refer to Sec~\ref{sec:ablation} for a detailed analysis.}
\label{tab:ablation}
\end{table*}

==> tables/benchmark.tex <==
\begin{table*}[t]
\small
    \centering
   \setlength\tabcolsep{2pt}% 调整列间距
    \begin{tabular}{lcccccccccccccccccc}
        \toprule
     %\multirow{2}{*}{Method}  & \multirow{2}{*}{\#Param} & \multirow{2}{*}{Data} & \multirow{2}{*}{VQA Data} & \multicolumn{2}{c}{POPE-R} & \multicolumn{2}{c}{POPE-P} & \multicolumn{2}{c}{POPE-A} & \multicolumn{10}{c}{MME}\\
     \multirow{2}{*}{Method} & \multirow{2}{*}{VQA Data} & \multicolumn{6}{c}{POPE} & \multicolumn{11}{c}{MME}\\
        \cmidrule(lr){3-8} \cmidrule(lr){9-19} & & AC-R & PR-R & AC-P & PR-P & AC-A & PR-A & EX & CT & PO & CO & PT & CE & SC & LM & AT & OC & Overall \\
        \midrule
        MiniGPT-4 & - & 77.8 & 75.4 & 68.3 & 64.3 & 66.6 & 62.45 & 68.3 & 55.0 & 43.3 & 75.0 & 41.8 & 54.4 & 71.8 & 54.0 & 60.5 & 57.5 & 581.7 \\
        MM-GPT & - & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & - & - & - & - & - & - & - & - & - & - & 654.7 \\
        IB-LLM & -  & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 775.8\\
        IB-LLM & -  & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 775.8\\
        InstructBLIP & - & 88.7 & 85.0 & 81.4 & 75.1 & 74.4 & 67.7 & 185 & 143.3 & 66.7 & 153.3 & 123.8 & 101.2 & 153.0 & 79.8 & 134.3 & 72.5 & 1212.8 \\
        Otter & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 1292.3 \\
        Muffin & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 1281.0 \\
        BLIP-2 & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 1293.8 \\
        \midrule 
        LLaVA & - & 54.4 & 52.3 & 52.4 & 51.3 & 50.8 & 50.4 & - & - & - & - & - & - & - & - & - & - & 502.8 \\
        Ours-PM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & 1289.2 \\
        Ours-RM & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        Ours & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        
        \bottomrule
    \end{tabular}
    \caption{\small{\textbf{Quantitative Results on POPE and MME benchmark.} We compare the Large Vision Language Model using the Vicuna backbone.}}
    \label{tab:pope}

\vspace{-4mm}
\end{table*}
\end{table*}

==> tables/benchmark_v2.tex <==
\begin{table*}[t]
\small
    \centering
   \setlength\tabcolsep{5pt}% 调整列间距
    \begin{tabular}{lcccccccccccccc}
        \toprule
     %\multirow{2}{*}{Method}  & \multirow{2}{*}{\#Param} & \multirow{2}{*}{Data} & \multirow{2}{*}{VQA Data} & \multicolumn{2}{c}{POPE-R} & \multicolumn{2}{c}{POPE-P} & \multicolumn{2}{c}{POPE-A} & \multicolumn{10}{c}{MME}\\
     \multirow{2}{*}{Method} & \multirow{2}{*}{\#Param} & \multirow{2}{*}{VQA Data} & \multicolumn{6}{c}{POPE} & \multicolumn{6}{c}{MMViG}\\
        \cmidrule(lr){4-9} \cmidrule(lr){10-15} & & & AC-R & PR-R & AC-P & PR-P & AC-A & PR-A & HL & CS & CA & AA & RA & Overall \\
        \midrule
        MiniGPT-4 & 7B & - & 77.8 & 75.4 & 68.3 & 64.3 & 66.6 & 62.45 & - & - & - & - & - & -  \\
        MM-GPT & & $\checkmark$ & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & 50.0 & - & - & - & - & - & -  \\
        IB-LLM & & $\checkmark$  & - & - & - & - & - & - & - & - & - & - & - & - \\
        InstructBLIP & 13B & $\checkmark$ & 88.7 & 85.0 & 81.4 & 75.1 & 74.4 & 67.7 & - & - & - & - & - & - \\
        Otter & & $\checkmark$ & - & - & - & - & - & - & - & - & - & - & - & - \\
        Muffin & & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        BLIP-2 & 13B & $\checkmark$ & & - & - & - & - & - & - & - & - & - & - & -  \\
        \midrule 
        LLaVA & 7B & - & 54.4 & 52.3 & 52.4 & 51.3 & 50.8 & 50.4 & - & - & - & - & - & - \\
        Ours-PM & 7B & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        Ours-RM & 7B & - & - & - & - & - & - & - & - & - & - & - & - & - \\
        Ours & 7B & - & - & - & - & - & - & - & - & - & - & - & - & -  \\
        
        \bottomrule
    \end{tabular}
    \caption{\small{\textbf{Quantitative Results on POPE and MMViG benchmark.}}}
    \label{tab:pope}

\vspace{-4mm}
\end{table*}

==> tables/gpt4v-backup.tex <==
\begin{table*}[t]
    \centering
    \setlength\tabcolsep{7pt}
    \begin{tabular}{l|ccc|ccccccc|c}
        \toprule
        \textbf{Method} & \textbf{LLM} & \textbf{\#Param} & \textbf{Data} &  \textbf{EA} & \textbf{CA} & \textbf{AA} & \textbf{RA} & \textbf{RL} & \textbf{CR} & \textbf{DL} & \textbf{Overall} \\
        \midrule
        OpenFlamingo & Vicuna & 13B & - & & & & & & & & \\
        MiniGPT-4 & - & 7B & 5k & & & & & & & & \\
        Shikra & Vicuna & 13B & 5.5M & & & & & & & & \\
        InstructBLIP & Vicuna & 7B & 1.2M & & & & & & & & \\
        InstructBLIP & Vicuna & 13B & 1.2M & & & & & & & & \\
        BLIP-2 & Vicuna & 13B & - & & & & & & & & \\
        \midrule
        LLaVA & Vicuna & 7B & 158K & & & & & & & & \\
        LLaVA & Vicuna & 13B & 158K & & & & & & & & \\
        \rowcolor{gray!20} Ours-GD & Vicuna & 7B & 158K & & & & & & & & \\
        \rowcolor{gray!20} Ours-RM & Vicuna & 7B & 172K & & & & & & & & \\
         \rowcolor{gray!20} Ours-All & Vicuna & 7B & 172K & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{EA: Existence Accuracy; CA: Counting Accuracy; AA: Attribute Accuracy; RA: Relation Accuracy; RL: Relevance; CR: Creativity; DL: Detail Level.}}
    \label{tab:mn40}
%\vspace{-0.1in}
\end{table*}

==> tables/gpt4v.tex <==
\begin{table*}[t]
    \centering
    \setlength\tabcolsep{7pt}
    \begin{tabular}{l|ccc|ccccccc|c}
        \toprule
        \textbf{Method} & \textbf{LLM} & \textbf{\#Param} & \textbf{Data} &  \textbf{HL} & \textbf{CP} & \textbf{CA} & \textbf{AA} & \textbf{RA} & \textbf{CR} & \textbf{RL} & \textbf{Overall} \\
        \midrule
        OpenFlamingo & Vicuna & 13B & - & & & & & & & & \\
        MiniGPT-4 & - & 7B & 5k & & & & & & & & \\
        Shikra & Vicuna & 13B & 5.5M & & & & & & & & \\
        InstructBLIP & Vicuna & 7B & 1.2M & & & & & & & & \\
        InstructBLIP & Vicuna & 13B & 1.2M & & & & & & & & \\
        InstructBLIP & Vicuna & 13B & 1.2M & & & & & & & & \\
        BLIP-2 & Vicuna & 13B & - & & & & & & & & \\
        \midrule
        LLaVA & Vicuna & 7B & 158K & & & & & & & & \\
        LLaVA & Vicuna & 13B & 158K & & & & & & & & \\
        \rowcolor{gray!20} Ours-GD & Vicuna & 7B & 158K & & & & & & & & \\
        \rowcolor{gray!20} Ours-RM & Vicuna & 7B & 172K & & & & & & & & \\
         \rowcolor{gray!20} Ours-All & Vicuna & 7B & 172K & & & & & & & & \\
        \bottomrule
    \end{tabular}
    \captionof{table}{\small{HL: Hallucination; CP: Completeness; CA: Counting Accuracy; AA: Attribute Accuracy; RA: Relation Accuracy; CR: Creativity; RL: Relevance.}}
    \label{tab:gpt4v}
%\vspace{-0.1in}
\end{table*}

==> tables/module_ablation.tex <==
\begin{table}[t]
\footnotesize
\centering
\setlength\tabcolsep{9pt}
\begin{tabular}{cccc}
        \toprule
         AT-RM & HF-RM & Refine & MMViG\\
        \midrule
        \cmark & - & - & 521.41 \\
        \cmark & - & \cmark & 536.59 \\
        - & \cmark & \cmark & 544.96 \\
        \cmark & \cmark & - & 551.87 \\
        \cmark & \cmark & \cmark & \textbf{575.31} \\
        \bottomrule
\end{tabular}

\caption{\textbf{Ablation studies on different components of our framework.}}
\vspace{-5pt}
\label{tab:ab_model}
\end{table}

==> tables/rebuttal_llavarlhf.tex <==
\begin{table}[h]
    \centering
    %\footnotesize
    \vspace{-7pt}
    \scriptsize
    \begin{tabular}{cccc}
        %\toprule
         & MMHal-Bench &  POPE (Avg F1 Score) \\
        \midrule
        $\text{LLaVA}_{\text{7B}}$ & 1.3 & 76.0 \\
        $\text{LLaVA-RLHF}_{\text{7B}}$ & 1.4 \textcolor[rgb]{0,0.6,0}{(+0.1)} & 78.2 \textcolor[rgb]{0,0.6,0}{(+2.2)}\\
        Ours &  \textbf{1.6} \textcolor[rgb]{0,0.6,0}{(+0.3)} & \textbf{83.5} \textcolor[rgb]{0,0.6,0}{(+7.5)} \\
        %\bottomrule
    \end{tabular}
    %\caption{}
    \vspace{-12pt}
    \label{tab:fps} 
\end{table}


